Real-Time Safe Bipedal Robot Navigation using Linear Discrete Control Barrier Functions

Safe navigation in real-time is an essential task for humanoid robots in real-world deployment. Since humanoid robots are inherently underactuated thanks to unilateral ground contacts, a path is considered safe if it is obstacle-free and respects the robot's physical limitations and underlying dynamics. Existing approaches often decouple path planning from gait control due to the significant computational challenge caused by the full-order robot dynamics. In this work, we develop a unified, safe path and gait planning framework that can be evaluated online in real-time, allowing the robot to navigate clustered environments while sustaining stable locomotion. Our approach uses the popular Linear Inverted Pendulum (LIP) model as a template model to represent walking dynamics. It incorporates heading angles in the model to evaluate kinematic constraints essential for physically feasible gaits properly. In addition, we leverage discrete control barrier functions (DCBF) for obstacle avoidance, ensuring that the subsequent foot placement provides a safe navigation path within clustered environments. To guarantee real-time computation, we use a novel approximation of the DCBF to produce linear DCBF (LDCBF) constraints. We validate the proposed approach in simulation using a Digit robot in randomly generated environments. The results demonstrate that our approach can generate safe gaits for a non-trivial humanoid robot to navigate environments with randomly generated obstacles in real-time.

==> sections/background.tex <==
% \section{Section}

% Section text here. 

% \subsection{Subsection Heading Here}
% Subsection text here.

% \subsubsection{Subsubsection Heading Here}
% Subsubsection text here.
\section{Method}

In this section, we first review the LIP model, a common bipedal model [], and present a corresponding LIP model-based MPC optimization problem to find the optimal controls for bipedal robots. Moreover, considering the safety factors, we also designed corresponding kinematic and environmental constraints based on the robot's walking characteristics. 
The goal is to provide a safe guaranteed obstacle avoidance path and generate corresponding controls for bipedal robots. 

\subsection{Linear Inverted Pendulum Model}
There are two expressions of the LIP model. One is the expression of the model in the local frame, which represents the CoM states of the robot in coordinates with the current stance foot as the origin []. In this expression, the coordinates need to be updated, and states also need to be transformed as the stance foot changes. The other expression is in the global frame, where both robot states and stance foot positions are expressed on a fixed coordinate system []. In our algorithm, we use the LIP model expressed in the global frame. This choice is because fixed coordinates can more easily represent obstacle information in the environment, such as CBFs. Moreover, using fixed coordinates prevents the robot's state from becoming discrete due to the frequent transformation needed to change coordinates.

\begin{figure}
\centering
\vspace{2mm}
    \begin{subfigure}[b]{0.48\linewidth}
         \centering
        \includegraphics[trim={7cm 0cm 8cm 0cm},clip,width=\linewidth]{Figures/LIP_ori.png}
         \caption{}
         \label{fig:LIP_ori}
     \end{subfigure}
     \begin{subfigure}[b]{0.47\linewidth}
         \centering
        \includegraphics[trim={8cm 0.5cm 7cm 0cm},clip,width=\linewidth]{Figures/LIP_dis_x.png}
         \caption{}
         \label{fig:LIP_x_dis}
     \end{subfigure}
     \begin{subfigure}[b]{1\columnwidth}
         \centering
        \includegraphics[trim={4cm 0cm 4cm 0cm},clip,width=\columnwidth]{Figures/LIP_new.png}
         \caption{}
         \label{fig:LIP_new}
     \end{subfigure}
\caption{\small{The Linear Inverted Pendulum Model. (a). The inverted pendulum locomotion in the x direction with a constant CoM height in the continuous time domain. (b). The inverted pendulum locomotion in the x direction with a fixed walking time duration. (c). The terminal states of the LIP model $\mathbf{x}_{k+1}$ switch its stance foot from $(f_{x_k}, f_{y_k})$ to $(f_{x_{k+1}}, f_{y_{k+1}})$ in the global frame}
} 
\vspace{-3.5mm}
\end{figure}

We use $H$ to denote the height of CoM of the robot and we assume the height of the robot would not change during the walking process. $g$ to denote the acceleration of gravity. Then the robot motion in the x-axis direction is:
\begin{align}
    \ddot{p_x} &= \frac{g}{H}(p_x-f_x)
\end{align}
where $p_x$ denotes the CoM position of the robot and $f_x$ denotes the stance foot displacement, see \figref{fig:LIP_ori}. We assume each walking step takes the same time duration $T$, and the robot is now at the beginning of time interval$[kT, (k+1)T)$. We define the initial position and velocity of the robot at the time $kT$ in the x-axis direction as $p_{x_k}$ and $v_{x_k}$, and the discrete foot displacement required at the current time is $f_{x_k}$, see \figref{fig:LIP_x_dis}. Then the closed-form solution of the robot terminal states at the end of the period is:
\begin{align}
\label{eq:x_dir_dynamics}
    \begin{bmatrix} p_{x_{k}+1} \\ v_{x_{k+1}} \end{bmatrix} =  \mathbf{A_d}
    \begin{bmatrix} p_{x_k} \\ v_{x_k} \end{bmatrix}
    + \mathbf{B_d}
    f_x
\end{align}
with: 
\begin{equation}
\label{eq:matrix_small}
\begin{aligned}
    \mathbf{A_d} &\coloneqq \left[ {\begin{array}{cc}
    \cosh(\beta t) & \frac{\sinh(\beta t)}{\beta}\\
   \beta\sinh(\beta t)  & \cosh(\beta t)
    \end{array} } \right]\\
    \mathbf{B_d} &\coloneqq \begin{bmatrix} 1-\cosh(\beta t) \\-\beta\sinh(\beta t) \end{bmatrix}
\end{aligned}
\end{equation}
where $\beta = \sqrt{g/H}$\\
For the 3D-LIP model, the motion in the y-axis direction is identical to the x-axis, and the turning of the heading is entirely independent of LIP control. Thus, we introduced an independent heading angle state $\theta$ and turning control $\phi$ to facilitate the subsequent construction of kinematic constraints.
The robot CoM states can be denoted as 
\begin{align}
\label{eq:states}
    \mathbf{x} \coloneqq [p_x, v_x, p_y, v_y, \theta]^T
\end{align}
and robot control:
\begin{align}
\label{eq:controls}
    \mathbf{u} \coloneqq [f_x, f_y, \phi]^T
\end{align}

Then, the modified 3D-LIP dynamics from step $k$ to step $k+1$ phase can be written as:

\begin{align}
\label{eq:system_dynamics}
    \mathbf{x}_{k+1} =  \mathbf{A}
    \mathbf{x}_k
    + \mathbf{B}\mathbf{u}_k
\end{align}
with: 
% \begin{equation}
% \label{eq:system_matrix}
% \begin{aligned}
%     \mathbf{A} &\coloneqq \begin{bmatrix}
%     \mathbf{A_d} & \mathbf{0}_{2\times2} & \mathbf{0}_{2\times1}\\
%     \mathbf{0}_{2\times2}& \mathbf{A_d} & \mathbf{0}_{2\times1}\\
%     \mathbf{0}_{1\times2} &  \mathbf{0}_{1\times2} & 1
%     \end{bmatrix} \\
%     \mathbf{B} &\coloneqq \begin{bmatrix} 
%     \mathbf{B_d} & \mathbf{0}_{2\times1} & \mathbf{0}_{2\times1}\\
%     \mathbf{0}_{2\times1} & \mathbf{B_d}  & \mathbf{0}_{2\times1}\\
%     0 & 0 & 1
%     \end{bmatrix}
% \end{aligned}
% \end{equation}
\begin{equation}
\label{eq:system_matrix}
\begin{aligned}
    \mathbf{A} &\coloneqq \begin{bmatrix}
    \mathbf{A_d} & \mathbf{0} & \mathbf{0}\\
    \mathbf{0}& \mathbf{A_d} & \mathbf{0}\\
    \mathbf{0} &  \mathbf{0} & 1
    \end{bmatrix} \\
    \mathbf{B} &\coloneqq \begin{bmatrix} 
    \mathbf{B_d} & \mathbf{0} & \mathbf{0}\\
    \mathbf{0} & \mathbf{B_d}  & \mathbf{0}\\
    0 & 0 & 1
    \end{bmatrix}
\end{aligned}
\end{equation}
where the dimension of matrix $A$ is $5\times5$, the dimension of matrix $B$ is $5\times3$.\\
Since the states and controls of the robot are defined in the global frame, the terminal states at the end of the previous time interval can be directly used as the initial states starting at the next time interval, see \figref{fig:LIP_new}, for example, $\mathbf{x}_{k+1}$ would be the initial states for time interval $[(k+1)T, (k+2)T)$.





\subsection{Discrete Control Barrier Function}
Consider robot discrete states $\mathbf{x}_k \in \mathcal{X}$ is the system state with $\mathcal{X}\subseteq \mathbb{R}^n$ being the state space, and $\mathbf{u}_k \in \mathcal{U}$ is the discrete control input with $\mathcal{U}\subseteq \mathbb{R}^m$ being the control space. If there exists a continuous and differentiable function $h: \mathbb{R}^n \rightarrow \mathbb{R}$, the safety set $\mathcal{C}$ of the system may be defined as []:
\begin{equation}
\label{eq:safety-set}
\begin{aligned}
    \mathcal{C} &= \{\mathbf{x}_k\in \mathbb{R}^n |h(\mathbf{x}_k) \geq 0\},\\
    \partial\mathcal{C} &= \{\mathbf{x}_k\in \mathbb{R}^n |h(\mathbf{x}_k) = 0\}.
\end{aligned}
\end{equation}
Then, $h$ is a control barrier function (CBF) if it follows the condition in the discrete-time domain for all $\mathbf{x}_k)\in\mathcal{C}$:
\begin{equation}
\label{eq:cbf_off}
\begin{aligned}
    \exists \text{ } \mathbf{u}_k &\text{ s.t. } \bigtriangleup h(\mathbf{x}_k, \mathbf{u}_k) \geq -\gamma(h(\mathbf{x}_k))
\end{aligned}
\end{equation}
where $\bigtriangleup h(\mathbf{x}_k, \mathbf{u}_k) \coloneqq h(\mathbf{x}_{k+1}) - h(\mathbf{x}_k)$, and $\gamma$ is a class $\kappa$ function that satisfies $0 < \gamma(h(x)) \leq h(x)$. In the discrete domain, $\gamma$ can be also a scalar that $0 < \gamma \leq 1$. So, the equation can be written as:
\begin{equation}
\label{eq:cbf_simp}
\begin{aligned}
    \exists \text{ } \mathbf{u}_k &\text{ s.t. } h(\mathbf{x}_{k+1}) + (\gamma - 1)h(\mathbf{x}_k) \geq 0
\end{aligned}
\end{equation}
Since the discrete control $\mathbf{u}_k$ is affine in (9 equ), it can be the DCBF constraint in MPC or QP to synthesize safe control.
